Finding hypergraph immersion is fixed-parameter tractable

Immersion minor is an important variant of graph minor, defined through an injective mapping from vertices in a smaller graph $H$ to vertices in a larger graph $G$ where adjacent elements of the former are connected in the latter by edge-disjoint paths. Here, we consider the immersion problem in the emerging field of hypergraphs. We first define hypergraph immersion by extending the injective mapping to hypergraphs. We then prove that finding a hypergraph immersion is fixed-parameter tractable, namely, there exists an $O(N^6)$ polynomial-time algorithm to determine whether a fixed hypergraph $H$ can be immersed in a hypergraph $G$ with $N$ vertices. Additionally, we present the dual hypergraph immersion problem and provide further characteristics of the algorithmic complexity.

==> refs.bbl.tex <==
\bibitem{q-netw-memory_mlpnk24}Meng, X., Lo Piparo, N., Nemoto, K. \& Kovács, I. Quantum Networks Enhanced by Distributed Quantum Memories. {\em Preprint}. pp. arXiv:2403.16367 (2024)
\bibitem{embed-fix-param-tract_gkmw11}Grohe, M., Kawarabayashi, K., Marx, D. \& Wollan, P. Finding Topological Subgraphs Is Fixed-Parameter Tractable. {\em Proceedings Of The Forty-Third Annual ACM Symposium On Theory Of Computing}. pp. 479-488 (2011)
\bibitem{fix-param-tract_df92}Downey, R. \& Fellows, M. Fixed-Parameter Intractability. {\em [1992] Proceedings Of The Seventh Annual Structure In Complexity Theory Conference}. pp. 36-49 (1992)
\bibitem{graph-theor-appl}Gross, J. \& Yellen, J. Graph Theory and Its Applications. (CRC Press,2005)
\bibitem{hypergr-theor-introd}Bretto, A. Hypergraph Theory: An Introduction. (Springer,2013)
\bibitem{mader_m67}Mader, W. Homomorphieeigenschaften und mittlere Kantendichte von Graphen.. {\em Mathematische Annalen}. \textbf{174} pp. 265-268 (1967)
\bibitem{robertson-seymour_rs10}Robertson, N. \& Seymour, P. Graph Minors XXIII. Nash-Williams' Immersion Conjecture. {\em Journal Of Combinatorial Theory, Series B}. \textbf{100}, 181-205 (2010)
\bibitem{hypergr-percolation_bd23}Bianconi, G. \& Dorogovtsev, S. The Theory of Percolation on Hypergraphs. {\em ArXiv Preprint}. pp. arXiv:2305.12297 (2023)
\bibitem{wagner1937minor}Wagner, K. Über eine Eigenschaft der ebenen Komplexe. {\em Math. Ann.}. \textbf{114} pp. 570-590 (1937)
\bibitem{lovasz2005minor}Lovász, L. Graph minor theory. {\em Bulletin Of The American Mathematical Society}. \textbf{43}, 75-86 (2005)
\bibitem{robertson2004wagner}Robertson, N. \& Seymour, P. Graph Minors. XX. Wagner's conjecture. {\em Journal Of Combinatorial Theory, Series B}. \textbf{92}, 325-357 (2004), Special Issue Dedicated to Professor W.T. Tutte
\bibitem{robertson1995paths}Robertson, N. \& Seymour, P. Graph Minors .XIII. The Disjoint Paths Problem. {\em Journal Of Combinatorial Theory, Series B}. \textbf{63}, 65-110 (1995)
\bibitem{fellows1988linear}Fellows, M. \& Langston, M. Nonconstructive tools for proving polynomial-time decidability. {\em J. ACM}. \textbf{35}, 727-739 (1988)
\bibitem{lovasz2019graphs}Lovász, L. Graphs and geometry. (American Mathematical Soc.,2019)
\bibitem{buchheim2014drawing}Buchheim, C., Chimani, M., Gutwenger, C., Jünger, M. \& Mutzel, P. Crossings and planarization. {\em Handbook Of Graph Drawing And Visualization}. pp. 43-79 (2014)
\bibitem{fellows1992app}Fellows, M. \& Langston, M. On Well-Partial-Order Theory and Its Application to Combinatorial Problems of VLSI Design. {\em SIAM J. Discrete Math.}. \textbf{5}, 117-126 (1992)
\bibitem{tian2024quanimmersion}Tian, Y., Liu, Y. \& Meng, X. Quantum Networks: from Multipartite Entanglement to Hypergraph Immersion. {\em Preprint}. pp. arXiv:2406.13452 (2024)
\bibitem{q-netw-route_p19}Pirandola, S. End-to-End Capacities of a Quantum Communication Network. {\em Communications Physics}. \textbf{2}, 1-10 (2019)
\bibitem{multipartite-q-netw-route_sb23}Sutcliffe, E. \& Beghelli, A. Multiuser Entanglement Distribution in Quantum Networks Using Multipath Routing. {\em IEEE Transactions On Quantum Engineering}. \textbf{4} pp. 1-15 (2023)
\bibitem{q-netw-route_pkttjbeg19}Pant, M., Krovi, H., Towsley, D., Tassiulas, L., Jiang, L., Basu, P., Englund, D. \& Guha, S. Routing Entanglement in the Quantum Internet. {\em Npj Quantum Information}. \textbf{5}, 25 (2019)
\bibitem{q-netw-route_lphnm20}Lo Piparo, N., Hanks, M., Nemoto, K. \& Munro, W. Aggregating Quantum Networks. {\em Physical Review A}. \textbf{102}, 052613 (2020)
\bibitem{path-percolation_mhrk24}Meng, X., Hao, B., Ráth, B. \& Kovács, I. Path Percolation in Quantum Communication Networks. {\em ArXiv Preprint}. pp. arXiv:2406.12228 (2024)
\bibitem{multipartite-q-netw_ctpv21}Contreras-Tejada, P., Palazuelos, C. \& De Vicente, J. Genuine Multipartite Nonlocality Is Intrinsic to Quantum Networks. {\em Physical Review Letters}. \textbf{126}, 040501 (2021)
\bibitem{multipartite-q-netw_wxkhlhgsp20}Wang, M., Xiang, Y., Kang, H., Han, D., Liu, Y., He, Q., Gong, Q., Su, X. \& Peng, K. Deterministic Distribution of Multipartite Entanglement and Steering in a Quantum Network by Separable States. {\em Physical Review Letters}. \textbf{125}, 260506 (2020)
\bibitem{multipartite-commun-q-netw}Meignant, C. Multipartite Communications over Quantum Networks. (Sorbonne Université,2021)
\bibitem{multipartite-q-netw_hpe19}Hahn, F., Pappa, A. \& Eisert, J. Quantum Network Routing and Local Complementation. {\em Npj Quantum Information}. \textbf{5}, 1-7 (2019)
\bibitem{bianconi2021hyper}Bianconi, G. Higher-Order Networks. (Cambridge University Press,2021)
\bibitem{klamt2009biology}Klamt Hypergraphs and Cellular Networks. {\em PLOS Computat. Biol.}. \textbf{5}, 1-6 (2009,5)
\bibitem{jost2019hyperL}Jost, J. \& Mulas, R. Hypergraph Laplace operators for chemical reaction networks. {\em Adv. Math.}. \textbf{351} pp. 870-896 (2019)
\bibitem{taramasco2010collab}Taramasco, C. Academic team formation as evolving hypergraphs. {\em Scientometrics}. \textbf{85}, 721-740 (2010)
\bibitem{krumov2011collab}Krumov, L., Fretter, C., Müller-Hannemann, M., Weihe, K. \& M. Hütt Motifs in co-authorship networks and their relation to the impact of scientific publications. {\em Eur. Phys. J. B}. \textbf{84}, 535-540 (2011)
\bibitem{Kwang2023core}Lee, J., Goh, K., Lee, D. \& Kahng, B. (k, q)-core decomposition of hypergraphs. {\em Chaos Solitons Fractals}. \textbf{173} pp. 113645. (2023)
\bibitem{berge1973hyper}Berge, C. Graphs and hypergraphs. (North-Holland,1973)

